Plotting in a Formally Verified Way

An invaluable feature of computer algebra systems is their ability to plot the graph of functions. Unfortunately, when one is trying to design a library of mathematical functions, this feature often falls short, producing incorrect and potentially misleading plots, due to accuracy issues inherent to this use case. This paper investigates what it means for a plot to be correct and how to formally verify this property. The Coq proof assistant is then turned into a tool for plotting function graphs using reliable polynomial approximations. This feature is provided as part of the CoqInterval library.

==> eptcsdata.tex <==
\providecommand{\firstpage}{39}
\providecommand{\publicationstatus}{A. Paskevich, J. Proen\c{c}a (Eds.): Formal Integrated\\
Development Environment 2021 (F-IDE 2021)\\
EPTCS 338, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.338.6}{10.4204/EPTCS.338.6}}
\pdfoutput=1

